Randomized Linear Algebra Approaches to Estimate the Von Neumann Entropy of Density Matrices

Thevon Neumann entropy, named after John von Neumann, is an extension of the classical concept of entropy to the field of quantum mechanics. From a numerical perspective, von Neumann entropy can be computed simply by computing all eigenvalues of a density matrix, an operation that could be prohibitively expensive for large-scale density matrices. We present and analyze three randomized algorithms to approximate von Neumann entropy of {real} density matrices: our algorithms leverage recent developments in the Randomized Numerical Linear Algebra (RandNLA) literature, such as randomized trace estimators, provable bounds for the power method, and the use of random projections to approximate the eigenvalues of a matrix. All three algorithms come with provable accuracy guarantees and our experimental evaluations support our theoretical findings showing considerable speedup with small loss in accuracy.

==> notation.tex <==
\section{Notation}\label{sxn:notation}

We will focus on finite-dimensional function (state) spaces. In this setting, the density matrix $\bR$ represents the statistical mixture of pure states and has the form
%
\begin{equation}\label{eqn:R}
%
\bR = \sum_{i=1}^k p_i \bpsi_i \bpsi_i^T  \in \mathbb{R}^{n \times n}.
%
\end{equation}
%
The vectors $\bpsi_i \in \mathbb{R}^n$ represent the $k \leq n$ pure states and can be assumed to be pairwise orthogonal and normal (XXX IS THIS ALWAYS THE CASE OR JUST IN THE QUANTUM ENSEMBLE SETTING XXX) while the $p_i$'s correspond to the probability of each state and satisfy $p_i > 0$ and $\sum_{i=1}^k p_i = 1$. From a linear algebraic perspective, eqn.~(\ref{eqn:R}) can be rewritten as
%
\begin{equation}\label{eqn:R1}
%
\bR = \bPsi \bSigma_p \bPsi^T \in \mathbb{R}^{n \times n},
%
\end{equation}
%
where $\bPsi \in \mathbb{R}^{n \times k}$ is the matrix whose columns are the vectors $\bpsi_i$ and $\bSigma_p \in \mathbb{R}^{k \times k}$ is a diagonal matrix whose entries are the (positive) $p_i$'s. Given our assumptions for $\bpsi_i$, $\bPsi^T\bPsi=\bI$; also $\bR$ is positive semi-definite with its non-zero singular values equal to the $p_i$ and corresponding left/right singular vectors equal to the $\bpsi_i$'s; and $\trace{\bR}=\sum_{i=1}^k p_i = 1$. Notice that eqn.~(\ref{eqn:R1}) essentially reveals the (thin) SVD of $\bR$.

\noindent The Von Neumann entropy of $\bR$, denoted by $\mathcal{H}(\bR)$ is equal to
%
\begin{equation}\label{eqn:VN}
%
\mathcal{H}(\bR) = -\sum_{i, p_i> 0} p_i \ln p_i = -\trace{\bR \ln \bR}.
%
\end{equation}
%
The second equality follows from the definition of matrix functions~\cite{Higham:2008}. More precisely, we overload notation and consider the full SVD of $\bR$, namely $\bR = \bPsi \bSigma_p \bPsi^T$, where $\bPsi \in \mathbb{R}^{n \times n}$ is an orthogonal matrix whose top $k$ columns correspond to the $k$ pure states and the bottom $n-k$ columns are chosen so that $\bPsi \bPsi^T = \bPsi^T \bPsi = \bI_n$. Here $\bSigma_p$ is a diagonal matrix whose bottom $n-k$ diagonal entries are set to zero. Let $h(x) = x \ln x$ for any $x>0$ and let $h(0)=0$. Then,
%
\begin{equation}
-\sum_{i, p_i> 0} p_i \ln p_i = -\trace{\bPsi h(\bSigma_{p}) \bPsi^T} = -\trace{h(\bR)} = -\trace{\bR \ln \bR}.
\end{equation}
%
In the above derivation, we used the cyclical property of the trace and the definition of $h(x)$. 
